Efficient Document Embeddings via Self-Contrastive Bregman Divergence Learning

Learning quality document embeddings is a fundamental problem in natural language processing (NLP), information retrieval (IR), recommendation systems, and search engines. Despite recent advances in the development of transformer-based models that produce sentence embeddings with self-contrastive learning, the encoding of long documents (Ks of words) is still challenging with respect to both efficiency and quality considerations. Therefore, we train Longfomer-based document encoders using a state-of-the-art unsupervised contrastive learning method (SimCSE). Further on, we complement the baseline method -- siamese neural network -- with additional convex neural networks based on functional Bregman divergence aiming to enhance the quality of the output document representations. We show that overall the combination of a self-contrastive siamese network and our proposed neural Bregman network outperforms the baselines in two linear classification settings on three long document topic classification tasks from the legal and biomedical domains.

==> tables/fewshot_scotus.tex <==
\begin{table}[h]
\centering
\begin{tabular}{lcc}
\toprule
 {\bf Model} & \microf & \macrof  \\
 \midrule
     Longformer_{\text{DA}} & \underline{54.9} & \underline{48.1}  \\     
     >> {\text{+SimCSE}} & 51.8 & 43.6  \\
     >> {\text{+ SimCSE + Bregman}} & \textbf{56.9} & \textbf{48.5} \\ 
\bottomrule
\end{tabular}
\caption{Test Results for all Longformer variants for SCOTUS. Best performance in Bold. The second-best score is underlined} 
\end{table}

==> tables/pooling.tex <==
\begin{table*}[h]
\centering
\begin{booktabs}{
  colspec = {lcccc},
  cell{1}{2,4} = {c=2}{c}, % multicolumn (column number=2, center alignment)
}
\toprule
  Models &   Longformer_{\text{DA + \ac{SimCSE}}} &      & Longformer_{\text{DA + \ac{SimCSE} + \ac{MLP}}}  &   \\
\midrule
       &  \mu\text{-}F1 &  m\text{-}F1 &  \mu\text{-}F1  & m\text{-}F1 \\
\cmidrule[lr]{2-3}\cmidrule[lr]{4-5} 
 Mean+Max Pooling & \textbf{78.3} & \textbf{70.6} &  \textbf{64.2} & \textbf{43.1} \\
 Mean Poolig & 76.9 & 68.1 & \underline{61.8} &  35.5 \\
  Max Pooling  & \underline{77.6} &  \underline{69.5} & 61.4 &36.1 \\ 
\code{[CLS]} Pooling & 77.1 & 69.5 &  61.0 & \underline{35.8} \\ 
%w/o Pooling & 75.4 & 66.7 & NA & NA\\
%No Classification Pooling & & & &\\
\bottomrule
\end{booktabs}
\caption{F1 performance of \gls{pooling} operators for \ac{SCOTUS}}
\label{tab:pool}
\end{table*}

==> tables/pooling_frozen_only.tex <==
\begin{table}[h]
\centering
\begin{booktabs}{
  colspec = {lcc},
  cell{1}{2,4} = {c=2}{c}, % multicolumn (column number=2, center alignment)
}
\toprule
  Models &    Longformer_{\text{DA + \ac{SimCSE} + \ac{MLP}}}  &   \\
\midrule
       &    \mu\text{-}F1  & m\text{-}F1 \\
\cmidrule[lr]{2-3}
 Mean+Max Pooling & \textbf{64.2} & \textbf{43.1} \\
 Mean Poolig & \underline{61.8} &  35.5 \\
  Max Pooling   & 61.4 &36.1 \\ 
\code{[CLS]} Pooling &  61.0 & \underline{35.8} \\ 
\bottomrule
\end{booktabs}
\caption{F1 performance of \gls{pooling} operators for \ac{SCOTUS}}
\label{tab:pool}
\end{table}
